Crowdsourcing the State of the Art(ifacts)

In any field, finding the "leading edge" of research is an on-going challenge. Researchers cannot appease reviewers and educators cannot teach to the leading edge of their field if no one agrees on what is the state-of-the-art. Using a novel crowdsourced "reuse graph" approach, we propose here a new method to learn this state-of-the-art. Our reuse graphs are less effort to build and verify than other community monitoring methods (e.g. artifact tracks or citation-based searches). Based on a study of 170 papers from software engineering (SE) conferences in 2020, we have found over 1,600 instances of reuse; i.e., reuse is rampant in SE research. Prior pessimism about a lack of reuse in SE research may have been a result of using the wrong methods to measure the wrong things.

==> response/response1-v2.tex <==
% 
\newpage
%\pagestyle{roman}
\setcounter{page}{1}
\section*{Response to Reviewers}
\subsection*{Associate Editor Comments}

 a) The methodology/metrics used to show the "unsatisfactory" nature of the current situation should be carefully justified. Both R2 and R3 raise serious concerns about how "reuse" was actually measured. If the authors can justify how they did it, that would really strengthen the paper. They also need make stronger construct validity argument (viz., what "reuse" is and why it matters. All reviewers seem to have trouble with this). 
 
 \noindent
\response{E.1}{We are very grateful for your thorough reviews with positive comments and detailed suggestions about our paper and research. We have made extensive changes to our paper based on your comments. This new version offers detailed notes
on how we measured reuse and how we double checked those measures (see the Kappa scores in Figure~\ref{results}b).}


b) The conceptual framework used by the authors to  structure the proposed solution for fixing the putative problem of "reuse" needs to be more clearly articulated, and supported. Supporting evidence ideally should come not ONLY from the authors' own experience with artifacts tracks.

 \noindent
\response{E.2}{We agree completely with your comment.
We agree that the  old version was far too
qualitative and 
``personal''. That older version   spent too much time on the artifact evaluation track material.~\\This new version, on the other hand is now more quantitative
and based on a summer of data collection that resulted in Figure~\ref{reuse}. The comments on the artifact evaluation track are now a minor part of the second half of the paper.
We hope you'll agree that this makes this new version
far more authoritative.}


c) The proposed remedy (Department of Reuse) should be more carefully justified, with arguments about why it would solve the problems raised. Both R2 and R3 are not convinced on this. 

 \noindent
\response{E.2}{We agree completely with your comment.
Our new introduction  (see {\S}1)
offers extensive arguments
about motivation and utility of our approach.}


d) Several editorial notes made by reviewers should be addressed. 

 \noindent
\response{E.3}{Thank you for those notes.
While this paper has been extensively revised,
where we have retained the older material,
we have applied those notes. 
Thank you for reviewing this version of our paper and we look forward to hearing from you.
~\\
\noindent
Sincerely,  \\ \\ 
Tim, Ben, Maria-Teresa, Neil}





\section{Reviewer 1}

\CHANGED{\em Please note that in response to feedback from ACM reviewers,
we have make extensive revisions to this draft. We thank you
for your detailed questions, below, and note that due
to those rewrites, some of your comments are now 
\underline{\bf OBE} (overcome by events).}
 

-       Page 1. Line 34. It would be helpful if the authors briefly explain (even in a footnote) how the replication and reproduction badges work. For example, if an artifact is replicated/reproduced months (or years) after the paper is published, will the paper be given the corresponding badge retroactively? 

\response{R1.1}{Thank you for that comment. Yes, that was not explained in the last draft. That has been fixed here.  \citeresp{1.1}.}

-       Page 1. Line 35. Did you check if those replicated/reproduced artifacts are the older ones? It would be interesting to know.

\response{R1.2}{Interesting question! 
The last draft did not check for that. But thanks to your comments, we can report that due to
failings in how reproduced results are reported,
{\em newer}
artifacts are  {\em more} likely to be reproduced
\citeresp{1.2}.}

-       Page 1. Lines 35-36. The paper reads “Note that this track record does not support the scientific process that generates trusted ideas that have been extensively used and tested”. What do you mean?

\response{R1.3}{OBE}

-       Page 2. Line 17. The authors use the word “reuse” throughout the paper several times (even the title). In this context, the term is misleading. There are “reusable”, “reproduced” and “replicated” badges. What are you exactly referring to? It is important to clarify the term.

 \response{R1.4}{Sorry about that confusion.
 The last draft was undisciplined in that respect.
 Here, in the body text, we now only use those terms once 
 \citeresp{1.4} where we say 
 ``not reused in replications or reproductions''. We think this
 distinguishes the terms adequately. But what do you think?}

-       Page 3. Lines 30-33 and Table 1. It surprises me that the authors suggest a flexible approach for artifact evaluation. Would not it be better to standardize how artifacts are evaluated? Perhaps the figure should be seen as the path to be followed in order to improve the artifact evaluation process, as the title of Table 1 seem to suggest? 

\response{R1.5}{\underline{\bf OBE}} 

-       Page 3. Lines 46-51. Another issue the authors should have in mind is that artifacts will be replicated/reproduced when it is fostered (or rewarded). The authors seem to take for granted (also in page 5) that people want to use artifacts, but their main problem is that they cannot be accessed.

\response{R1.6}{Good point, but is access the issue?
As mentioned above, we are finding hundreds of
previously undocumented examples  of reuse where the products
of paper1 are reused in a subsequent  paper2. So, at least from
what we are seeing, access is not the  issue.}

-       Page 5, line 38. What do you mean by “instantly”? Automatically? If so, perhaps it is not a good idea. Someone should check availability. Maybe you mean that no specific request from authors should be necessary? Please, clarify.

\response{R1.7}{\underline{\bf OBE}}

-       Page 6. Lines 31-40. In general, I think it is a very good idea to acknowledge replication and reproduction. Until we are not able to do so, it will be difficult to increase the replication/reproduction rate.

\response{R1.8}{We agree. It is the view of  this paper
that our current
reporting mechanism for reuse are missing many examples
of this  happening. We need to change that!  Hence, this paper.}

-       Figure 3 is impossible to read. Could you please, improve resolution? Perhaps increase its size?

\response{R1.9}{Thank 
you for that comment. In this draft we have take more care with the figures.}


OTHER COMMENTS: \CHANGED{{\em typos and references fixed as per your suggestion}}
 
 

\section{Reviewer 2}


\CHANGED{\em Please note that in response to feedback from ACM reviewers,
we have make extensive revisions to this draft. We thank you
for your detailed questions, below, and note that due
to those rewrites, some of your comments are now 
\underline{\bf OBE} (overcome by events).}


Overall, I am not sure what the aim of this paper is. The authors first examine (in a shallow way) AE processes in various communities and then proceed to
present a framework for characterizing them. Perhaps unsurprisingly, the framework has a technical and a social aspect. The authors claim that the technical issues are largely solved, so they focus on presenting some solutions
for the social aspects. They finish up by presenting a sketch for a tool to facilitate attribution for authors of reusable artifacts. 


\response{R2.1}{Thank you for your comment. You are right. We did not state our overall goal. Our new introduction  (see {\S}1)
offers extensive arguments
about motivation and utility of our approach.}

%I have several questions:

- Have the authors somehow validated the proposed framework?  Have the authors validated any of the proposed social issue solutions? I know
  that ROSE festivals have been running for some years now, but  what makes the authors sure that the "Department of Reuse" (DoR) will
  increase the overall reuse? 
  
\response{R2.2}{You are quite correct. It was incorrect
to use the ROSE initiative in that way and that has been dropped from this draft.
As to our other results
Figure~\ref{results} shows our validations studies. 
When we compute Kappa statistics
for the results of our readers,
we see $K=1$ (median). }.
 

Will more technology solve a (what the authors
  identify as) social issue?
  
\CHANGED{{\em Apologies for the socio/technical
distinctions made in the last draft. We have dropped that.
  } }
% \chn



- The authors claim that artifact discoverability is a big issue. Perhaps it is.
  But how does the DoR help solve that? If I need to find a dataset for my
  software transplantation study, how will the knowledge of "Tim Menzies" being
  the top reused artifact author help me in that?

\response{R2.4}{Good question! That was missing in the last
draft. Our new introduction lists 8 applications of these graphs.} 

- Why is Table 2 in the paper? Interesting as it is, I don't see how it fits the
  narrative.

\response{R2.5}{You are right. We have removed it}

- The authors claim that it is scandalous that after a decade of AECs only
  1/50th of the artifacts have been reused. I agree with the ratio, but not with
  the characterisation. Why is "scandalous"; Most of the artifacts I have seen
  in my tenure in AEC committees are replication packages, which are a must have
  for open science, but for which reuse is a happy accident.

\response{R2.6}{You are right- that was needlessly dramatic.  We have removed that wording.}

The paper, seen as a piece of text, has been clearly rushed and is not ready for
publication. There are several spelling and grammatical mistakes.

\response{R2.7}{Apologies! We have carefully proofread this version.}




\section{Reviewer 3}


\CHANGED{\em Please note that in response to feedback from ACM reviewers,
we have make extensive revisions to this draft. We thank you
for your detailed questions, below, and note that due
to those rewrites, some of your comments are now 
\underline{\bf OBE} (overcome by events).}




% This article draws attention to the problem of reproducibility in Software Engineering research.  Like many areas of science, SE research has been gripped by a "reproducibility crisis" in recent years.  The "crisis" is that many papers are published, but a relatively small percentage of those papers are reproducible.  One proposed remedy is a set of badge rewards from conferences to acknowledge papers that have published code and data artifacts to assist other researchers in reproducing or replicating the work.  This paper points out flaws in this "badges" remedy and points to potential solutions.

% This paper is a timely contribution to an important problem.  There is an overwhelming consensus that the reproducibility crisis does indeed affect SE research, and there is strong demand for a light-weight solution (i.e. one that can cover many papers while also not requiring too much extra time from reviewers).

% At the same time, this paper has a few issues which hold it back from being ready for publication, namely:

1) The central contention that "reusable is not reused" is not strongly validated.  The claim is supported by a web search for reusable artifact badges, and counting the percent of those badges that are Reproduced or Replicated.  There are a few problems with this simple approach.  

\CHANGED{Thank you for the care with which
you reviewed this paper. We are  very
interested in your remarks and have used
them to explicate much that  was  buried,
or overlooked, or confused in the earlier
draft.}

First, as the paper itself points out, it may take many years before a paper is reproduced in another paper, so the five-year time window may not be sufficient. 

\response{3.1}{\CHANGED{This is an interesting point. Your comment
caused us to look again at our data \citeresp{3.1}.
Figure~\ref{results}c tells us that most reuse comes from
very recent items.  Hence we believe that the issue
is not artifact maturity,  or time  to be recognize
but  rather how we recognize and reward reuse. Hence, 
this paper.
}}


Second, not all artifacts are intended to be reproduced.  For example, a data artifact may be used by other papers by not *reproduced* in the way that a code artifact is.

\response{3.2a}{\CHANGED{You make  another good point; i.e.
that it is now appropriate to reflect more
on  the  kinds of artifacts that we acknowledge
when we talk about ``reuse''. As discussed in this
paper, ``data'' is one of the six reuse types that we hunt for
in this study.  See \citeresp{3.2a}. }}

Third, badges may not be updated after being reproduced.  If a paper were published in, say, 2017 with a reproducible badge and then that paper were reproduced in 2021, it is not clear how often the old "reproducible" badge would be updated to "reproduced." 

\response{3.3}{\CHANGED{\em This is an area where we 
   are  in strong agreement. The badge  update
policy for ACM portal and IEEE Xplore
is clearly broken. The authors of this
paper have been personally  involved in numerous
SE conference  artifact   committees since 2017.
As such, we have awarded numerous replicated
and reproduced badges. None of these can be 
found in ACM portal or IEEE Xplore.}
}

Fourth, the badge system does not capture all replication and reproducibility.  Sometimes, artifacts are used to guide future researchers even if they are not directly reproduced using exactly what is provided in the artifact.  Consider again the hypothetical paper from 2017.  Four years later in 2021, many software versions and hardware details have changed, which may prompt new implementation.  However, that does not mean the old artifact is not reproducible -- it just means that enough details have changed that it is not practical to reuse, even if it is still useful as a guide.

\response{R3.4}{Interestingly, we have had the opposite experience. Recently we wrote up our reuse findings and made 20 submission to the FSE'21 artifacts evaluation committee.
As part of that process, we contacted
the authors who generated the reused artifact. In one case, that author noted that the reusing paper made an error in how they cited the reused artifact. Our FSE'21 submission
could fix that error. In summary: there
seems to be some added value in our work 
to clean up any small errata in reuse references.}

2) The paper makes several recommendations for artifacts tracks, but these recommendations seem disconnected from the key contention of the paper (reusable does not mean reused) and the proposed remedy via the website.  The recommendations seem to be based on the authors' experience with artifacts tracks, in which case these recommendations may be better suited to a position paper or public letter.  On the other hand, this paper could connect these recommendations more clearly to the over contention made by the paper.  One way to do this would be to provide more justification and, in this justification, draw more connections from each recommendation to the central contention of the paper.

\response{R3.5}{OBE. In this draft, we no longer propose fixing the artifact
evaluation process.}

3) The proposed "Department of Reuse" is interesting but it is not articulated well yet.  Basically the paper proposed a website to visualize different artifacts and papers that make use of those artifacts.  This website seems like it would be a good idea, but depends on yet more data curation and maintenance, which seems to run counter to the idea of minimizing workload on reviewers.  

\response{R3.6}{Good point.
Prompted by your question, we have looked into the effort
required to maintain our site, on an on-going basis. 
\citeresp{3.6}. The effort levels there are easily achievable.
Already this project has attracted the attention of researchers in  Hong Kong,  Turkey, 
Sweden, Finland and Australia. The data collected in this paper
was collected via their graduate students (see our footnote\#1).
We anticipate at least doubling that team as a result of the publication
of this CACM article.
And if that is not enough then   each of the authors  of this paper
run a 100+ person graduate class
once a year. If each year for the next five years,
those classes were assigned the homework described at the end of our Introduction, the we could cover the 2015-2025 conference papers from
the major SE events.  
}

% In conclusion, this paper contains useful information and targets an important problem, but is not quite ready for publication.  I sincerely hope to see the recommendations influence the research community, given the high value of reproducibility in SE.

 

==> response/response1.tex <==
% % 
% \newpage
% %\pagestyle{roman}
% \setcounter{page}{1}
% \section*{Response to Reviewers}
% \subsection*{Associate Editor Comments}

%  a) The methodology/metrics used to show the "unsatisfactory" nature of the current situation should be carefully justified. Both R2 and R3 raise serious concerns about how "reuse" was actually measured. If the authors can justify how they did it, that would really strengthen the paper. They also need make stronger construct validity argument (viz., what "reuse" is and why it matters. All reviewers seem to have trouble with this). 


% b) The conceptual framework used by the authors to  structure the proposed solution for fixing the putative problem of "reuse" needs to be more clearly articulated, and supported. Supporting evidence ideally should come not ONLY from the authors' own experience with artifacts tracks; if it is only that, then some arguments should be made about the generalizability, and also about potential external validity threats. 

% c) The proposed remedy (Department of Reuse) should be more carefully justified, with arguments about why it would solve the problems raised. Both R2 and R3 are not convinced on this. 

% d) Several editorial notes made by reviewers should be addressed. 



% \noindent
% \response{E.1}{We are very grateful for your thorough reviews with positive comments and detailed suggestions about our paper and research. We have made revisions to our paper based on your comments.~\\
% Below, we provide a summary of the main changes we made, and then we describe the additional changes, providing detailed responses to individual verbatim reviewer comments. We gloss over the summaries and comments that do not result in changes. 
% ~\\
% Thank you for reviewing this version of our paper and we look forward to hearing from you.
% ~\\
% \noindent
% Sincerely,  \\ \\ 
% Tim, Ben, Maria-Teresa, Neil}





% \section{Reviewer 1}
% -       Page 1. Line 34. It would be helpful if the authors briefly explain (even in a footnote) how the replication and reproduction badges work. For example, if an artifact is replicated/reproduced months (or years) after the paper is published, will the paper be given the corresponding badge retroactively? 

% \response{R1.1}{Thank you for that comment. Yes, that was not explained in the last draft.  \citeresp{1.1}.}

% -       Page 1. Line 35. Did you check if those replicated/reproduced artifacts are the older ones? It would be interesting to know.

% \response{R1.2}{Interesting question! 
% The last draft did not check for that. But thanks to your comments, we can report that due to
% failings in how reproduced results are reported,
% {\em newer}
% artifacts are  {\em more} likely to be reproduced
% \citeresp{1.2}.}

% -       Page 1. Lines 35-36. The paper reads “Note that this track record does not support the scientific process that generates trusted ideas that have been extensively used and tested”. What do you mean?

% \response{R1.3}{Apologies.  We have now repaired that
% confusing   sentence.\citeresp{1.3}.}

% -       Page 2. Line 17. The authors use the word “reuse” throughout the paper several times (even the title). In this context, the term is misleading. There are “reusable”, “reproduced” and “replicated” badges. What are you exactly referring to? It is important to clarify the term.

%  \response{R1.4}{Sorry about that confusion.
%  This draft takes  care to  note
%  that we  use ``reuse''
%  as the parent term for both ``reproduced'' and ``replicated'' \citeresp{1.4}}

% -       Page 3. Lines 30-33 and Table 1. It surprises me that the authors suggest a flexible approach for artifact evaluation. Would not it be better to standardize how artifacts are evaluated? Perhaps the figure should be seen as the path to be followed in order to improve the artifact evaluation process, as the title of Table 1 seem to suggest? 

% \response{R1.5}{Good point---but is now the time
% to standardize on how we review specific kinds of artifacts?
% Do we need more  experimentation
% before we  
% standardize? Perhaps. We
% are now part of an international consortium of researchers
% and graduate students whose  goal is to review the last
% decade  of papers looking for reuse in SE papers from main conferences such as:
% ICSE, FSE, ESEM, ASE, ICSME and MSR. For ICSE'22 (see \citeresp{R2.2b}). We are writing
% a submission listing  the hundreds of
% examples  of reused artifacts 
% found by that process.  We can report
% that (a)~many of those reused items
% are the `stepping stone'' reuse defined in \S \ref{dor} while 
% (b)~very
% few of those reused items fit the definitions of
% Figure~1. That is, if we had standardized on the definition
% of ``artifacts'', we would have  missed nearly all that reuse.} 

% -       Page 3. Lines 46-51. Another issue the authors should have in mind is that artifacts will be replicated/reproduced when it is fostered (or rewarded). The authors seem to take for granted (also in page 5) that people want to use artifacts, but their main problem is that they cannot be accessed.

% \response{R1.6}{Good point, but is access the issue?
% As mentioned above, we are finding hundreds of
% previously undocumented examples  of reuse where the products
% of paper1 are reused in a subsequent  paper2. So, at least from
% what we are seeing, access is not the  issue.}

% -       Page 5, line 38. What do you mean by “instantly”? Automatically? If so, perhaps it is not a good idea. Someone should check availability. Maybe you mean that no specific request from authors should be necessary? Please, clarify.

% \response{R1.7}{That was a poor choice of words. We mean
% that the human effort  in making that evaluation is minimal.
% \citeresp{1.7}.}

% -       Page 6. Lines 31-40. In general, I think it is a very good idea to acknowledge replication and reproduction. Until we are not able to do so, it will be difficult to increase the replication/reproduction rate.

% \response{R1.8}{We agree. It is the view of  this paper
% that our current
% reporting mechanism for reuse are missing many examples
% of this  happening. We need to change that!  Hence, this paper.}

% -       Figure 3 is impossible to read. Could you please, improve resolution? Perhaps increase its size?

% \response{R1.9}{Thank 
% you for that comment. We
% have updated that figure and, also, included in the figure text a pointer to a fill size  version of that graphic.}\


% OTHER COMMENTS:

% -       I think reference [9] is already published. I think I saw it in the EMSE TOC alert a month ago or so.\\
% -       Page 1, line 23.  “scientists re member”.\\
% -       Table 2. “ran a artifacts”.\\
% -       Page 6, line 32. “an other”.

% \response{R1.10}{Thanks, we have made these changes.}

% \section{Reviewer 2}
% Overall, I am not sure what the aim of this paper is. The authors first examine (in a shallow way) AE processes in various communities and then proceed to
% present a framework for characterizing them. Perhaps unsurprisingly, the framework has a technical and a social aspect. The authors claim that the technical issues are largely solved, so they focus on presenting some solutions
% for the social aspects. They finish up by presenting a sketch for a tool to facilitate attribution for authors of reusable artifacts. 


% \response{R2.1}{Thank you for your comment. You are right. We did not state our overall goal. That is now included in our new
%  new introduction. \citeresp{2.1}.}

% %I have several questions:

% - Have the authors somehow validated the proposed framework?  Have the authors validated any of the proposed social issue solutions? I know
%   that ROSE festivals have been running for some years now, but  what makes the authors sure that the "Department of Reuse" (DoR) will
%   increase the overall reuse? 
  
% \response{R2.2}{You are quite correct. That was missing from the prior paper.
% We would call our result "validated" if,  we can find reused
% artifacts that were missed by other
% artifact evaluation committees. Also,
% when we compute Kappa statistics
% for the results of our readers,
% we see $K>.7$ (which is the accepted
% standard) agreement on what people
% think is being reused. This paper offers
% preliminary results in that direction 
% \citeresp{2.2a} but not a detailed study.
% Note that such a detailed study is planned for ICSE'22. Whereas here, for the more generalist
% CACM audience, we focus more
% on the bigger picture rather than the detailed
% tedium of extensive statistical analysis. Furthermore, the two solutions DoR and ROSE are complementary, the first graphically representing the connections of where reuse occurs, and the second as moment where authors provide examples through short pitches of replication and reproduction}.
 

% Will more technology solve a (what the authors
%   identify as) social issue?
  
% \CHANGED{We are not sure that this paper
% is where we can answer that question.
% Speculatively, we say that it might be 
% possible 
% to (say) build a text mining classifier that 
% can find the examples of reuse we report here.
% But the certification of that classifier would require some ``ground truth'' of the kind
% we are collecting here
% \citeresp{2.2b}.  }
% \}
% % \chn

% - The authors claim that artifact discoverability is a big issue. Perhaps it is.
%   But how does the DoR help solve that? If I need to find a dataset for my
%   software transplantation study, how will the knowledge of "Tim Menzies" being
%   the top reused artifact author help me in that?

% \response{R2.4}{Good question!
% We envision a time,
% in the very near future, when Figure~\ref{dor} is a very dense graph. researchers in a field could then "walk backwards" across our links
% to find the artifacts that everyone is using.
% Then they can either look at the issues that that
% kind of artifact can address, or which it
% systematically misses. In either case,
% they have some basis for future research.}

% - Why is Table 2 in the paper? Interesting as it is, I don't see how it fits the
%   narrative.

% \response{R2.5}{We thought it served to broaden the scope of ``what is an artifact''. It shows that the kinds of things normally explored in artifact evaluation committees is only a small subset of what might be explored. If you think it fails in that aspect, we'd be more than willing to remove it}

% - The authors claim that it is scandalous that after a decade of AECs only
%   1/50th of the artifacts have been reused. I agree with the ratio, but not with
%   the characterisation. Why is "scandalous"; Most of the artifacts I have seen
%   in my tenure in AEC committees are replication packages, which are a must have
%   for open science, but for which reuse is a happy accident.

% \response{R2.6}{You are right- that was needlessly dramatic.  We have changed
% that. \citeresp{2.6}.}

% The paper, seen as a piece of text, has been clearly rushed and is not ready for
% publication. There are spelling and grammatical mistakes all over the place:
% just to indicate a few, p1 l24 "re member", p1 l25 "One way to encourage more
% science...", and p2 l31: "conduct severe tests".

% \response{R2.7}{Apologies! We have carefully proof read this version .}




% \section{Reviewer 3}
% % This article draws attention to the problem of reproducibility in Software Engineering research.  Like many areas of science, SE research has been gripped by a "reproducibility crisis" in recent years.  The "crisis" is that many papers are published, but a relatively small percentage of those papers are reproducible.  One proposed remedy is a set of badge rewards from conferences to acknowledge papers that have published code and data artifacts to assist other researchers in reproducing or replicating the work.  This paper points out flaws in this "badges" remedy and points to potential solutions.

% % This paper is a timely contribution to an important problem.  There is an overwhelming consensus that the reproducibility crisis does indeed affect SE research, and there is strong demand for a light-weight solution (i.e. one that can cover many papers while also not requiring too much extra time from reviewers).

% % At the same time, this paper has a few issues which hold it back from being ready for publication, namely:

% 1) The central contention that "reusable is not reused" is not strongly validated.  The claim is supported by a web search for reusable artifact badges, and counting the percent of those badges that are Reproduced or Replicated.  There are a few problems with this simple approach.  

% \CHANGED{Thank you for the care with which
% you reviewed this paper. We are  very
% interested in your remarks and have used
% them to explicate much that  was  buried,
% or overlooked, or confused in the earlier
% draft.}

% First, as the paper itself points out, it may take many years before a paper is reproduced in another paper, so the five-year time window may not be sufficient. 

% \respto{3.1}\CHANGED{This is an interesting point. Your comment
% caused us to look again at our data \citeresp{3.1}.
%  Looking into ACM Portal,
% we find that 67, 30, and 3\%  of the reproduced
% results are found 3, 6, and 9 years ago (respectively);
% i.e. more {\em recent} artifacts are {\em more} likely
% to be replicated. Hence we believe that the issue
% is not artifact maturity,  or time  to be recognize
% but  rather how we recognize and reward reuse. Hence, 
% this paper.
% }


% Second, not all artifacts are intended to be reproduced.  For example, a data artifact may be used by other papers by not *reproduced* in the way that a code artifact is.

% \respto{3.2}\CHANGED{You make  another good point; i.e.
% that it is now appropriate to reflect more
% on  the  kinds of artifacts that we acknowledge
% when we talk about ``reuse''.  
% FYI,   we
% are now part of an international consortium of researchers
% and graduate students whose  goal is to review the last
% decade  of papers looking for reuse in SE papers from relevant venues such as:
% ICSE, FSE, ESEM, ASE and MSR. For ICSE'22, we are writing
% a submission listing  the hundreds of
% examples  of reused artifacts 
% found by that process.  We can report
% that (a)~there are numerous examples
% of the kinds of reuse you mention above
% (the data artifact reuse)   while 
% (b)~very
% few of those data reused items fit the definitions of
% Figure~1.  
% }

% Third, badges may not be updated after being reproduced.  If a paper were published in, say, 2017 with a reproducible badge and then that paper were reproduced in 2021, it is not clear how often the old "reproducible" badge would be updated to "reproduced." 

% \respto{3.3}\CHANGED{This is an area where we 
% seem  more in agreement. The badge  update
% policy for ACM portal and IEEE Xplore
% is clearly broken. The authors of this
% paper have been personally  involved in numerous
% SE conference  artifact   committees since 2017.
% As such, we have awarded numerous replicated
% and reproduced badges. None of these can be 
% found in ACM portal or IEEE Xplore.
% {\em We urgently need to change the way we are reporting reuse.}.
% Hence, this paper. 
% }

% Fourth, the badge system does not capture all replication and reproducibility.  Sometimes, artifacts are used to guide future researchers even if they are not directly reproduced using exactly what is provided in the artifact.  Consider again the hypothetical paper from 2017.  Four years later in 2021, many software versions and hardware details have changed, which may prompt new implementation.  However, that does not mean the old artifact is not reproducible -- it just means that enough details have changed that it is not practical to reuse, even if it is still useful as a guide.

% \response{R3.1}{Interestingly, we have had the opposite experience. Recently we wrote up our reuse findings and made 20 submission to the FSE'21 artifacts evaluation committee.
% As part of that process, we contacted
% the authors who generated the reused artifact. In one case, that author noted that the reusing paper made an error in how they cited the reused artifact. Our FSE'21 submission
% could fix that error. In summary: there
% seems to be some added value in our work 
% to clean up any small errata in reuse references.}

% 2) The paper makes several recommendations for artifacts tracks, but these recommendations seem disconnected from the key contention of the paper (reusable does not mean reused) and the proposed remedy via the website.  The recommendations seem to be based on the authors' experience with artifacts tracks, in which case these recommendations may be better suited to a position paper or public letter.  On the other hand, this paper could connect these recommendations more clearly to the over contention made by the paper.  One way to do this would be to provide more justification and, in this justification, draw more connections from each recommendation to the central contention of the paper.

% \response{R3.2}{XXX}

% 3) The proposed "Department of Reuse" is interesting but it is not articulated well yet.  Basically the paper proposed a website to visualize different artifacts and papers that make use of those artifacts.  This website seems like it would be a good idea, but depends on yet more data curation and maintenance, which seems to run counter to the idea of minimizing workload on reviewers.  The paper should clarify the key objectives of the website and better connect those objectives to specific problems listed earlier in the paper.

% \response{R3.3}{Good point.
% Please see our new notes in the introduction. }

% % In conclusion, this paper contains useful information and targets an important problem, but is not quite ready for publication.  I sincerely hope to see the recommendations influence the research community, given the high value of reproducibility in SE.

 
